Understanding Dynamic Tactile Sensing for Liquid Property Estimation

Humans perceive the world by interacting with objects, which often happens in a dynamic way. For example, a human would shake a bottle to guess its content. However, it remains a challenge for robots to understand many dynamic signals during contact well. This paper investigates dynamic tactile sensing by tackling the task of estimating liquid properties. We propose a new way of thinking about dynamic tactile sensing: by building a light-weighted data-driven model based on the simplified physical principle. The liquid in a bottle will oscillate after a perturbation. We propose a simple physics-inspired model to explain this oscillation and use a high-resolution tactile sensor GelSight to sense it. Specifically, the viscosity and the height of the liquid determine the decay rate and frequency of the oscillation. We then train a Gaussian Process Regression model on a small amount of the real data to estimate the liquid properties. Experiments show that our model can classify three different liquids with 100% accuracy. The model can estimate volume with high precision and even estimate the concentration of sugar-water solution. It is data-efficient and can easily generalize to other liquids and bottles. Our work posed a physically-inspired understanding of the correlation between dynamic tactile signals and the dynamic performance of the liquid. Our approach creates a good balance between simplicity, accuracy, and generality. It will help robots to better perceive liquids in different environments such as kitchens, food factories, and pharmaceutical factories.

==> problem.tex <==
\section{Liquid Properties Estimation}
\label{sec: problem}
\joe{I don't like this title. Any ideas?}
\wenzhen{I think it makes more sense to put this back to the 'model' section. You can put it as 'III-A Overview' though}

Given a bottle of liquid, we aim to estimate the viscosity and volume of the liquid using only tactile sensors.
In general, solving this problem includes two steps: initiating the dynamics of the liquid-container by an activation motion, and estimating liquid properties using the collected dynamic tactile signal. Most approaches \cite{chen2016learning} \cite{8593838} \cite{saal} focus on the second step and design various data-driven approaches to estimate liquid properties.
Instead of estimating liquid properties in a purely data-driven way, our insight is to solve the problem by understanding and modeling the received dynamic tactile signal using physics. In fact, our approach complements physics-based models with data-driven models, and seeks to leverage the strengths of both: we model the simple physics principles and use data to learn the complicated physics we could not model.

A key novelty of our approach is the way we activate the system and collect dynamic tactile signals to prevent dealing with complicated dynamics. While shaking the liquid-container is the most popular activation motion, it causes complex, nonlinear dynamics like turbulence. Inspired by the importance of step response to system characterization, we command the robot to perform an ``unit step input": laterally perturb the liquid-container and then actively hold it still. The key is to collect dynamic tactile signal only in the ``hold still" stage, where the system dynamics is much simpler and the signal is cleaner (Fig. \ref{fig:fig1}d).

 %We specifically target the following properties: liquid viscosity, and liquid volume (quantified as the height of the liquid). We initiate the dynamics of the liquid-container by moving it with an activation motion and use the collected dynamic tactile signal to estimate liquid properties.
%In general, solving this task requires deciding on: how to estimate liquid properties using the collected dynamic tactile signal and what activation motion to perform to initiate the dynamics of the liquid-container. %choose to activate the liquid-container by shaking it, and estimate liquid properties in a purely data-driven way.
%Since these two steps are coupled, we start by considering the way to estimate liquid properties by dynamic tactile signals.
%While most approaches \cite{chen2016learning} \cite{8593838} \cite{saal} intuitively choose to initiate the liquid-container by shaking it, this activates complex dynamics like turbulence and complicates the liquid properties estimation approach

%Instead of estimating liquid properties in a purely data-driven way, our insight is to first understand and model the received dynamic tactile signal using physics. Our approach finds a synergetic balance between physics-based and data-driven models: we model the simple physics principles we know and use data to learn the complicated physics we could not model.  

\yifan{what's the difference betwen "shaking" and "laterally perturb"?}\joe{Shaking is a back-and-forth process and need to control the speed. Lateral perturbing just need an impulse or so.}
%This activation motion results in simpler dynamics and clean signal (Fig. \ref{fig:fig1}d).
\yifan{maybe define "activation motion" here? And how does activation motion relate to the task}
%The dynamics of the activated liquid-container system governs the dynamic tactile signal we received. 

